Explicit Visual Prompting for Low-Level Structure Segmentations

We consider the generic problem of detecting low-level structures in images, which includes segmenting the manipulated parts, identifying out-of-focus pixels, separating shadow regions, and detecting concealed objects. Whereas each such topic has been typically addressed with a domain-specific solution, we show that a unified approach performs well across all of them. We take inspiration from the widely-used pre-training and then prompt tuning protocols in NLP and propose a new visual prompting model, named Explicit Visual Prompting (EVP). Different from the previous visual prompting which is typically a dataset-level implicit embedding, our key insight is to enforce the tunable parameters focusing on the explicit visual content from each individual image, i.e., the features from frozen patch embeddings and the input's high-frequency components. The proposed EVP significantly outperforms other parameter-efficient tuning protocols under the same amount of tunable parameters (5.7% extra trainable parameters of each task). EVP also achieves state-of-the-art performances on diverse low-level structure segmentation tasks compared to task-specific solutions. Our code is available at: https://github.com/NiFangBaAGe/Explicit-Visual-Prompt.

==> figs/exp.tex <==

\newcommand\wwthree{0.3\textwidth}
\newcommand\hhthree{0.3\textwidth}

\begin{figure*}[t]
\centering
\includegraphics[width=0.3\linewidth]{figs/exp/CAISA_F1.png}
\includegraphics[width=0.3\linewidth]{figs/exp/ISTD_BER.png}
\includegraphics[width=0.3\linewidth]{figs/exp/DUT_FMeasure.png}
\caption{Mask Ratio.}
\label{fig:mask_ratio}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.3\linewidth]{figs/exp/CAISA_Filter.png}
\includegraphics[width=0.3\linewidth]{figs/exp/ISTD_Filter.png}
\includegraphics[width=0.3\linewidth]{figs/exp/DUT_Filter.png}
\caption{Filter.}
\label{fig:filter}
\end{figure*}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

